Motion Planning for Quadrupedal Locomotion: Coupled Planning, Terrain Mapping and Whole-Body Control

Planning whole-body motions while taking into account the terrain conditions is a challenging problem for legged robots since the terrain model might produce many local minima. Our coupled planning method uses stochastic and derivatives-free search to plan both foothold locations and horizontal motions due to the local minima produced by the terrain model. It jointly optimizes body motion, step duration and foothold selection, and it models the terrain as a cost-map. Due to the novel attitude planning method, the horizontal motion plans can be applied to various terrain conditions. The attitude planner ensures the robot stability by imposing limits to the angular acceleration. Our whole-body controller tracks compliantly trunk motions while avoiding slippage, as well as kinematic and torque limits. Despite the use of a simplified model, which is restricted to flat terrain, our approach shows remarkable capability to deal with a wide range of non-coplanar terrains. The results are validated by experimental trials and comparative evaluations in a series of terrains of progressively increasing complexity.

==> src/decoupled_planning.tex <==
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% 2345678901234567890123456789012345678901234567890123456789012345678901234567890
% 1         2         3         4         5         6         7         8
% %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% ******************************************************************************
% Decoupled motion and foothold planning
% ******************************************************************************
\section{Decoupled motion and foothold planning}\label{sec:decoupled_planning}
Natural locomotion over challenging terrain requires simultaneous computation of
footstep sequences, body movements and locomotion behaviors, i.e. coupled
planning. In this section, we split the planning and control problem into a set
of sub-problems, following a decoupled planning strategy. First, we plan a
sequence of footholds by planning an approximate body path
(\Cref{sec:foothold_planning}). The approximate body path is computed from a
sequence of planned body actions (\Cref{sec:body_action_planning}). Then we
choose locally the footholds locations (\Cref{sec:foothold_sequence_planning}).
Finally, we generate a body trajectory that ensures dynamic stability and
achieve the planned foothold sequence (\Cref{sec:com_traj_generation}). % We achieve a
% compliance execution by combining a virtual model with a floating-base inverse
% dynamic controllers (\Cref{sec:decoupled_execution}).
% 
% TODO --> maybe for introduction
% In the literature there are few coupled planner methods 
% \citep{Tassa2010,Mordatch2012a,Posa2013,Dai2014}. One of the main
% problems with such approaches is that the search space grows quickly and searching becomes
% unfeasible, especially for systems that need solutions in real-time. In
% contrast, we use a lattice representation (i.e. body movement primitives) for
% planning foothold sequence. Our hierarchical foothold planner increases the
% versatility of the body movements (e.g. discretized yaw-changing movements
% instead of continuous changes) compared to state-of-the-art approaches
% \citep{Kolter2008b,Vernaza2009,Kalakrishnan2009}. We reduce the computation time
% using a terrain-aware heuristic function which estimates the cost-to-go. We
% generate a \gls{com} trajectory that ensures dynamic stability and needs no
% knowledge of a predefined gait. For that, it checks if the next swing leg is
% diagonally opposite of the current swing leg. If so, the disjoint support
% triangles require a four-leg support phase for the optimization to find a
% solution. Both, the foothold and motion planners, increase the versatility of
% the planned motions compared to previous works. Furthermore, our framework
% builds online the terrain costmap and computes online the foothold sequence.
\Cref{fig:decoupled_framework} shows an overview of our decoupled motion and
foothold planning framework for dynamic legged locomotion over challenging
terrain.
%
All the material presented in this section has been previously published in
different works \citep{Mastalli2016,Winkler2015}. 

\begin{figure}[!tb]
	\centering
	\includegraphics[width=0.98\columnwidth]{figs/decoupled_planning/framework_overview-compressed.pdf}
	\caption[An overview of the perception, planning and control framework]{
	Overview of our decoupled motion and foothold planning framework
	\citep{Mastalli2015,Winkler2015}. The foothold planner first computes a
	sequence of body action and then selects the foothold locations $\mathbf{F}$
	around an action-specific foothold region. The foothold sequence is planned
	according the terrain information (i.e. terrain costmap and heightmap). Then
	the motion planner uses the planned footholds to generate dynamic whole-body
	motions ($\mathbf{x}^d, \mathbf{\dot{x}}^d, \mathbf{\ddot{x}}^d$). Finally, the
	desired motion is compliantly executed by using a combination of feed-forward
	and feedback terms.}
	\label{fig:decoupled_framework}
\end{figure}


\subsection{Foothold planning}\label{sec:foothold_planning}
This section describes the foothold planner, consisting of two main elements:
the \textit{body action planner} that decides the general direction of movement
through actions, and the \textit{local foothold planner} that chooses specific
footholds around those actions.

The overall task is to plan online an appropriate sequence of footholds
$\vc{F}$ that allows the robot to traverse a challenging terrain toward a body
goal state $(x,y,\theta)$. To accomplish this, our foothold planner first
computes a sequence of body action and then selects the foothold locations
around an action-specific foothold region. It searches a bounded sub-optimal
body path, through a sequence of body actions, in a growing \textit{body-state
graph}. The body-state graph uses the explored action to select an appropriate
foothold region. We use this region to compute the body cost, or transition cost
between two nodes in the graph.


\subsubsection{Body action planning.}\label{sec:body_action_planning}
For planning a sequence of body actions over challenging terrain, we consider the
varying difficulty of the terrain areas, obstacles, types of actions, potential
leg collisions, potential body orientations and kinematic reachability. Thus,
given a terrain costmap (see \Cref{sec:terrain_costmap}), the body action
planner computes a sequence of body actions that maximize the
\textit{cross-ability} of the terrain. The cross-ability describes how desirable
is a determined body path in terms of the terrain conditions. It is quantified
by computing a body cost along the path. The body action plans are computed by
searching over a \textit{body-state graph} that is built using a set of
predefined body movement primitives. \gls{aras} is used to find the optimal
action sequence \citep{Likhachev2004}. Our terrain-aware heuristic function
helps to achieve better performance by guiding the search efficiently.

\begin{figure}%[!tb]
	\centering
	\includegraphics[width=0.98\columnwidth]{figs/decoupled_planning/body_action_planning_v2}
	\caption[A sketch of the body action graph]{
	Sketch of the body action graph. The objective is to find a sequence of
	actions $\vc{a}$ from the current body state ${\vc{s}=(x,y,\theta)}$ to the
	goal state $\vc{g}$, that minimizes the accumulated body costs
	$c(\vc{s},\vc{a})$. For simplicity only three possible actions are shown,
	namely move left ($\vc{a}^l$), right ($\vc{a}^r$) and forward ($\vc{a}^f$). The
	optimal action sequence \{$\vc{a}^l, \vc{a}^r, \dots, \vc{a}^r$\} is
	obtained through a tree search as is shown in red.}
	\label{fig:body_action_graph}
\end{figure}


\paragraph{Graph construction:}
The \textit{body-state graph} is constructed using a lattice-based adjacency
model. The lattice representation is a discretization of the action space
into a set of feasible body movements. The body-state graph represents the
transition between different body-states (nodes) and it is defined as a tuple,
$\mathcal{G} = (\mathcal{S},\mathcal{E})$, where each node $\vc{s} \in
\mathcal{S}$ represents a \textit{body-state} and each edge $\vc{e} \in
\mathcal{E} \subseteq \mathcal{S} \times \mathcal{S}$ defines a feasible
transition from $\vc{s}$ to $\vc{s'}$ (see \cref{fig:body_action_graph}). The
body-state $(x,y,\theta)$ represents the 2D position and yaw angle,
respectively. Each edge represents a body movement primitives (i.e. a body
action). Each body movement primitive ensures feasibility along an appropriate
footstep region. Additionally, these footstep regions are defined to increase
the triangular support areas, improving the execution of the whole-body plan.

Given a body-state query, we construct dynamically the graph $\mathcal{G}$,
through a predefined set of body movement primitives, since the associated cost
of transition $c_{body}(\vc{s},\vc{s'})$ depends on the current and next states
(or current state and action). The associated cost of every transition is
computed using the footstep regions, as is shown in \cref{fig:footstep_regions}.
Moreover, an entire graph construction could require a greater memory
pre-allocation and computation time than available onboard.
\fref{fig:graph_construction} shows the graph construction for the body action
planner. For every expansion, the footstep regions of \gls{lf} (brown squares),
\gls{rf} (yellow squares), \gls{lh} (green squares) and \gls{rh} (blue squares)
legs are computed given a body action. For more details about the graph search
see \citep{Mastalli2015}.

\begin{figure}%[!b]%[!tb]
	\centering
 	\includegraphics[width=0.85\columnwidth]{figs/decoupled_planning/footstep_regions}
 	\caption[Different footstep search regions according to the body action]{
 	Different footstep search regions according to the body action.
 	These footstep regions ensure the feasibility of the plan. Moreover, these
 	predefined regions increase the triangular support areas, improving the
 	execution of the whole-body plan. The brown, yellow, green and blue squares
 	represent the footstep search regions for \gls{lf}, \gls{rf}, \gls{lh} and
 	\gls{rh} feet, respectively.}
	\label{fig:footstep_regions}
\end{figure}

\begin{figure}[b]
	\centering
	\includegraphics[width=0.9\columnwidth]{figs/decoupled_planning/graph_construction.pdf}
	\caption[Illustration of graph construction of the least-cost path]{
	Illustration of graph construction of the least-cost path. The associated cost
	of every transition $c_{body}(\vc{s},\vc{s'})$ is computed using the footstep
	regions. For every expansion, the footstep regions of \gls{lf} (brown squares),
	\gls{rf} (yellow squares), \gls{lh} (green squares) and \gls{rh} (blue squares)
	are computed according to a certain body action.}
	\label{fig:graph_construction}
\end{figure}

\paragraph{Body cost:}
The body cost describes how \textit{desirable} it is for the robot to be at a
specific area of the terrain. By evaluating a sequence of such areas and their
costs along a body path, we can understand how difficult/desirable it would be
to cross it. This cost is designed to maximize the \textit{cross-ability} of the
terrain while minimizing the path length. The body cost function $c_{body}$ is a
linear combination of: terrain cost $c_t$, action cost $c_a$, potential leg
collision cost $c_{pc}$, and potential body orientation cost $c_{po}$. Thus the
cost of the transition from the body state $\vc{s}$ to $\vc{s'}$ is defined as
follows:
\begin{eqnarray}\label{eq:body_cost}\nonumber
	c_{body}(\vc{s},\vc{s'}) = w^b_t c_t(\vc{s}) + w_a
	c_a(\vc{s},\vc{s'}) \\
	+ w_{pc} c_{pc}(\vc{s}) + w_{po} c_{po}(\vc{s}),
\end{eqnarray}
where $w^b_t$, $w_a$, $w_{pc}$ and $w_{po}$ are the weights of terrain, action,
potential leg and collision costs, respectively.

For a given body state $\vc{s}$, the terrain cost $c_t$ is evaluated by
averaging the best $n$-footsteps terrain cost values around the foothold regions
of a nominal stance (nominal foothold positions). The action cost $c_{a}$ is
defined by the user according to the desirable actions of the robot (e.g. it is
preferable to make diagonal body movements than lateral ones). The potential leg
collision cost $c_{pc}$ is computed by searching potential obstacles in the
predefined workspace region of the foothold, e.g. near to the shin of the robot.
In fact, a potential shin collision is detected around a predefined region,
which depends on the configuration of each leg as shown in
\fref{fig:shin_collision}. This cost is proportional to the height defined
around the footstep plane, where red bars represent collision elements.
Finally, the potential body orientation $c_{po}$ is estimated by fitting a plane
in the possible footsteps around the nominal stance for each leg.

\begin{figure}%[b]
	\centering
	\includegraphics[width=0.7\columnwidth]{figs/decoupled_planning/potential_shin_collision}
	\caption[Computation of the potential shin collision]{
	Computation of the potential shin collision. The potential shin collisions are
	detected around a predefined region (red bars). The computed cost is
	proportional to the height defined (red lines) around the footstep plane
	(dashed black lines), where blue height differences do not contribute to the
	cost.}
	\label{fig:shin_collision}
\end{figure}

% \paragraph{Reducing the search space} TODO ---> maybe in the result section
% Decoupling the foothold planning problem into body action and foothold planning
% avoids the combinatorial search space explosion. This allows us to compute plans
% quickly ($\sim$\unit[1.5]{sec} on average for our benchmark trials which
% around 40 steps), and develop a closed-loop foothold planning approach that can
% deal with changes in the environment. We represent the search space using an
% abstract graph which is embedded in the Euclidean space. Our lattice
% representation uses a set of predefined body movement primitives that allows us
% to apply a set of rules that ensure feasibility and reduce the search space.
% 
% The body movement primitives are defined as 3D \textit{actions}, $a \in (\Delta
% x, \Delta y, \Delta \theta)$, of the body that discretize the search space. We
% define a set of different movements such as: forward and backward, diagonal,
% lateral and yaw-changing motions.

% \paragraph{Ensuring feasibility}\label{sec:ensuring_feasibility}
% Our lattice representation allows the robot to search a body-action plan
% according to a set of predefined body movement primitives. The body movement
% primitives also define nominal feet positions and accordingly transitions  (see
% \cref{fig:footstep_regions}). This way we chose nominal positions that undertake
% to increase the supporting polygon, and as a consequence, to improve the
% conditions of the subsequent quadratic optimization problem for the whole-body
% motion generation phase that follows in \Cref{sec:com_traj_generation}.

\paragraph{Heuristic function:}\label{sec:terrain_aware_heuristic}
The heuristic function guides the search toward promising body actions,
improving the efficiency of the search. Heuristic-based search algorithms
require that the heuristic function is admissible and consistent. Often, when
planning within Cartesian spaces, heuristic functions estimate the cost-to-go by
computing the Euclidean distance to the goal. Such heuristic functions do not
consider the terrain difficulty and geometry, and often under or over-estimate
the cost-to-go considerably. In contrast, our terrain-aware heuristic function
considers the terrain geometry and produces an estimated cost-to-go according to
the already acquired knowledge of the environment. It estimates the cost-to-go
(i.e. body actions) by averaging the terrain cost locally and estimating the
number of footsteps to the goal:
\begin{equation}\label{eq:heuristic_function}
	h(\vc{s}) = -\bar{R}\mathcal{F}(\|\vc{g}-\vc{s}\|),
\end{equation}
where $\bar{R}$ is the average cost and $\mathcal{F}(\|\vc{g}-\vc{s}\|)$
is the function that estimates the number of footholds from the current state
$\vc{s}$ to the goal state $\vc{g}$.

% \paragraph{Ensuring online planning}
% Open-loop, or offline, planning approaches fail to deal adequately with changes
% in the environment. In real scenarios, the robot has a limited range of
% perception that makes open-loop planning approaches unreliable. Closed-loop
% planning considers the changes in the terrain conditions, and uses predictive
% terrain conditions for non-perceived regions, improving the robustness of the
% plan. Dealing with re-planning and updating of the environment information
% requires that the information is managed in an efficient search exploration of
% the state space. We manage to reduce the computation time of building a costmap
% by computing the cost values from a voxelized map\footnote{A voxelized map is a
% volumetric discretization of the environment, i.e. a grid discretization in 3D
% space} of the environment. Additionally, we (re-)plan and update the information
% using \gls{aras} \citep{Likhachev2004}. \gls{aras} ensures provable bounds on
% sub-optimality, depending on the definition of the heuristic function. Note that
% the terrain-aware heuristic function guides the search according to terrain
% conditions.


\subsubsection{Local foothold planning.}\label{sec:foothold_sequence_planning}
Given the desirable body action plan, the local foothold planner computes the
sequence of footholds that reflects the intention of the body action. A local
greedy search procedure selects the optimal footstep target around an
action-specific foothold region, as shown in \cref{fig:footstep_regions}. We
evaluate the foothold target through a \textit{footstep cost}. For more details
about how the foothold search algorithm see \citep{Mastalli2015}.

\paragraph{Footstep cost:}
The footstep cost describes how desirable is a foothold target, given a body
action $\vc{a}$. The purpose of this cost function is to maximize the
locomotion stability given a candidate set of footsteps. The footstep cost
$c_{footstep}$ is a linear combination of: terrain cost $c_t$, support triangle
cost $c_{st}$, shin collision cost $c_c$ and body orientation cost $c_o$.
The cost of certain footstep $\vc{f}^e$ is defined as follows:
\begin{eqnarray}\label{eq:footstep_cost}\nonumber
	c_{footstep}(\vc{f}^e) = w^f_t c_t(\vc{f}^e) + w_{st}
	c_{st}(\vc{f}^e) \\
	+ w_{c} c_{c}(\vc{f}^e) + w_{o} c_{o}(\vc{f}^e),
\end{eqnarray}
where $\vc{f}^e$ defines the Cartesian position of the foothold target $e$
(foot index). We consider as end-effectors: the \gls{lf}, \gls{rf}, \gls{lh} and
\gls{rh} feet of \gls{hyq}.

The terrain cost $c_t$ is computed from the terrain cost value of the
candidate foothold, i.e. using the terrain costmap (see
\Cref{sec:terrain_costmap}). The support triangle cost $c_{st}$ depends on the
in-radii of the triangle formed by the current footholds and the candidate one.
As in the body cost computation, we use the same predefined collision region
around the candidate foothold. Finally, the body orientation cost $c_{o}$ is
computed using the plane formed by the current footsteps and the candidate one.
We calculate the orientation of the robot from this plane.



\subsection{Motion planning}\label{sec:com_traj_generation}
The planned body trajectory ensures that the robot is \emph{dynamically
stable} at every time step. As in the approach \citep{Kalakrishnan2010b},
the \gls{com} trajectory respects dynamic constraints without explicitly
generating a \gls{cop} trajectory. We extend this approach by enabling
\emph{completely unconstrained}\footnote{Not constrained to any specific gait
sequence (e.g. the McGhee gait), the legs can swing in any order.} swing-leg
sequences and adaptation of four-leg support times according to the robot's
motion.

For a \gls{com} trajectory to be feasible it must be continuous and double
differentiable. This way we avoid steps in accelerations that produce
discontinuous torques. It is crucial for the inverse dynamics computation, and
furthermore can damage the hardware and affect stability. Ensuring that the
robot's \gls{com} follows a fifth-order polynomial as:
\begin{equation}
  x(t) = a_xt^5 + b_xt^4 + c_xt^3 + d_xt^2 + e_xt + f_x
  \label{eq:poly}
\end{equation}
satisfies both requirements. Note that $x(t)$ refers to the position of the
\gls{com} at time $t$, and the lateral component (i.e. $y(t)$) is equally
described. Generating an optimal \gls{com} trajectory represented by one spline
can thus be reduced to find a set of optimal polynomial coefficients:
\begin{equation}
	\mathbf{q} = \{a_x \ldots f_x, a_y \ldots f_y\} \in \mathbb{R}^{12}.
\end{equation}

Describing the \gls{com} trajectory for multiple steps by one polynomial restricts
the movement. Hence, we describe the trajectory as a spline composed of multiple
quintic polynomials. At each spline junction we require the last state ($t=T_i$) of
spline $i$ to be equal to the first state ($t=0$) of the next spline $i\!+\!1$
as:
\begin{equation}
  (\vc{x}, \dot{\vc{x}}, \ddot{\vc{x}})_{t=T_i}^i = (\vc{x}, \dot{\vc{x}},
  \ddot{\vc{x}})_{t=0}^{i+1},
  \label{eq:equality}
\end{equation}
where $\vc{x} = [x, y, z]$ is the \gls{com} position and $\vc{p} = [p_x,
p_y, p_z]$ is the \gls{cop} position.

This ensures double differentiability and continuity of the trajectory, required
by the floating-base inverse dynamics used in the whole-body controller (see
\Cref{sec:execution}).


\subsubsection{Dynamic stability.}\label{subsec:cop_stability}
To execute the footholds, a body trajectory must be found that ensures a
stable stance at all time instances. In case of slow and static movements the
\gls{com} must be inside the current support polygon, i.e. the polygon formed by
the legs in stance. We generate \emph{dynamic} movements with large body
accelerations using the cart-table model \citep{Kajita2003} described by:
\begin{equation}
  p_x = x - \frac{z \ddot{x}} {\ddot{z} + g_0},
  \label{eq:cop}
\end{equation}
where $p_x$ and $x$ are the position of the \gls{cop} and the \gls{com}
respectively, $z$ describes the height of the robot with respect to the feet,
$\ddot{z}$ is the vertical acceleration of the body and $g_0$ represents the
gravitational acceleration.

Dynamic stability is achieved by keeping the \gls{cop} inside the current
support triangle instead of the \gls{com} (\cref{fig:cart_and_com}). This
constraint is modeled by expressing the support triangle by three lines $\vc{l}$
of the form $px + qy + d = 0$. The \gls{cop} is considered to be \emph{inside} a
support triangle, if the following conditions\footnote{The direction of the
inequality sign depends on the line convention.} are met at every sampling
interval:
\begin{equation}
  p_l p_x + q_l p_y + r_l > 0 \quad \text{ for } l=1,2,3.
  \label{eq:line}
\end{equation}

In reality there exist discrepancies between the \gls{cop} position from
the model and the real robot. Additionally, desired body trajectories cannot be
perfectly tracked as modeling, sensing and actuation inaccuracies are hard to
avoid. Therefore, it is best to avoid the border of stable configurations by
shrinking the support triangles by a stability margin $r$ (see
\cref{fig:supp_triangle}). Because of this, there is no continuous \gls{cop}
trajectory when switching between diagonally opposite swing legs, as the support
triangles are disjoint. We allow a transition period (four-leg support phase)
during which the \gls{cop} is only restricted to the shrunk support
\emph{polygon} created by the four stance feet.
\begin{figure*}[tb]
	\centering
	\subfloat[]{\resizebox{0.25\textwidth}{!}{
		\includegraphics{figs/decoupled_planning/cart_table_model.pdf}}}
  	\quad\hspace{-0.4cm}
  	\subfloat[]{\resizebox{0.74\textwidth}{!}{
  		\includegraphics{figs/decoupled_planning/com_trajectory_exp.pdf}}}
 	\caption[The cart-table model]{
 	(\textit{a}) The cart-table model; the base of the table is formed
 	by the feet that are in stance (in contact) while this model assumes that all the
 	robot's mass is point-concentrated on the accelerating cart on top of the
 	table. (\textit{b}) The \gls{com} trajectory is represented by a series of
 	5\textsuperscript{th} order polynomials that are constrained to have
 	sequentially equal boundary values. At each (evaluated) point in time, we
 	constrain the \gls{cop} to lie inside the support polygon that the stance feet
 	form, thus the system is in a dynamically stable state.}
 	\label{fig:cart_and_com}
\end{figure*}

\begin{figure}[tb]
	\centering
	\includegraphics[width=0.85\columnwidth]{figs/decoupled_planning/supp_tr_disjoint}
	\caption[Disjoint support triangles due to the added stability margin $r$]{
	Disjoint support triangles due to the added stability margin $r$.
	When switching between swinging the \gls{lf} to \gls{rh} the \gls{cop} must
	move from the blue to the pink support triangle. Since all four feet are in
	stance during this phase, the \gls{cop} is only restricted by the red support
	polygon.}
  \label{fig:supp_triangle}
\end{figure}

\paragraph{Minimizing accelerations (cost function):}
In addition to moving in a dynamically stable way, the trajectory should
accelerate as little as possible during the execution period $T$. This increases
possible execution speed and reduces required joint torques. As in
\citep{Kalakrishnan2010b} this is achieved by adding a cost function of the
form:
\begin{equation}
  g = w_x \int_{0}^{T}\! \ddot{x}^2(t)\,dt + w_y\int_{0}^{T}\!
  \ddot{y}^2(t)\,dt
  \label{eq:cost_fun}
\end{equation}
to the quadratic program.

The directional weights $\mathbf{w}$ penalize sideways accelerations ($w_y =
1.5w_x$) more than forward-backward motions, since sideways motions are more
likely to cause instability. This torque-minimization function can also be
viewed as a regularization term. We solve the resulting convex \gls{qp} using a
freely available \gls{qp} solver, namely \textit{QuadProg++} \citep{quadprog}.

\paragraph{Irregular swing-leg sequences:}
We allow a \emph{completely irregular sequence} of steps for the \gls{cop}
optimization. Our trajectory generator needs no knowledge of a predefined gait.
For \emph{every} step it checks if the next swing leg is diagonally opposite of
the current swing leg. If so, the disjoint support triangles require a four-leg
support phase in the optimization. This allows a greater decoupling from the
foothold planner, which can generate swing leg sequences in any order useful for
the success of the behavior.

\paragraph{Feasible four-leg support time:}
In addition to inserting a four-leg support phase, the \emph{duration} $t_{4ls}$
of this phase affects the quality of locomotion. A \textit{too short} time
requires large accelerations that might cause slippage in the feet when executed.
A \textit{too long} time on the other hand reduces locomotion speed and can
oppose the natural dynamics of the system.

We adapt the four-leg support times according to the robot's motion using
$t_{4ls} = r \cdot t_{swing}$, where $r$ is the stability margin of the support
triangles, and $t_{swing}$ is the duration of a leg swing. This formulation
respects the movement of the robot to overcome the stability margins of
both support triangles. Furthermore, it complies to the body velocity imposed by
$t_{swing}$. The more accurate the \gls{cop} describes the dynamics of the
system, the smaller the margin $r$ can be chosen, effectively reducing the four
leg-support time and increasing locomotion speed. In case of perfect
correspondence between model and reality and perfect trajectory tracking, a
stability margin is not necessary. The four-leg support phase can be eliminated
($t_{4ls} = 0$), since the \gls{cop} can move smoothly between any
support triangle of the walking gait.


\subsubsection{Trunk attitude and swing-leg trajectory.}
To avoid kinematic limits the height of the robot follows the average height of
the stance legs, raised by a desired ground clearance. The body pitch adapts to
the difference between the height of the front and the hind legs, whereas the
body roll depends on the difference between the height of the left and the right
legs.

We adapt the swing leg trajectory based on the start and the goal foothold. If
the goal foothold lies higher than the start, we raise the lift height to avoid
collisions. Furthermore, we swing outward to avoid potential collisions, e.g.
with a stair step, while swinging up as in \citep{Winkler2014}. For steps on
flat ground the lift height is low with no outward motion to increase speed.



% \section{Control and Execution}\label{sec:decoupled_execution}
% Dynamic whole-body motions require orchestrated and precise actuation of all the
% joints. Simple PD joint position controllers do not suffice for such motions,
% especially when considering uncertainties in the environment and/or model
% inaccuracies. We use a control scheme (\cref{fig:decoupled_framework}) that
% combines a virtual model with a floating-base inverse dynamics controller.
% 
% After receiving an arbitrary sequence of footholds from the footstep planner,
% the whole-body motion generator calculates desired (feed-forward) accelerations
% $\vc{\ddot{x}}^d$ for the body and a virtual model (VM) control loop adds
% feedback accelerations $\vc{\ddot{x}}^{\!f\!b}$ should the robot deviate from
% the desired trajectory. The inverse dynamics produce the majority of the joint
% torques which are combined with a low-gain joint-space PD controller to
% compensate for possible model inaccuracies. The computed reference torques are
% then tracked by the low-level torque controller
% \citep{Boaventura2012a}\citep{Boaventura2012b}. Note that $\vc{x}$ describes the
% linear and rotational coordinates of the body as:
% \begin{equation}
%  \vc{x} = (\vc{x}_{cog}, \mx{R}_{b}),
%  \vc{\dot{x}} = (\vc{\dot{x}}_{com}, \boldsymbol{\omega}_b),
%  \vc{\ddot{x}} = (\vc{\ddot{x}}_{com}, \dot{\boldsymbol{\omega}}_b), 
% \end{equation}
% where $\mx{R}_b \in \Rnum^{3\times 3}$ is a coordinate rotation matrix
% representing the orientation of the base w.r.t. the world frame and
% $\boldsymbol{\omega}_b \in \Rnum^3$ is the angular velocity of the base.
% %
% %From the planned footholds a desired body trajectory and orientation is
% %generated (see \sref{sec:trajectory_generation}) at the position $\vc{x}^d = (\vc{x}_{cog}^d, \mx{R}_{b}^d)$, velocity $\vc{\dot{x}}^d = (\vc{\dot{x}}_{cog}^d$, $\vc{\omega}_b^d$) and acceleration  $\vc{\ddot{x}}^d = (\vc{\ddot{x}}_{cog}^d$, $\vc{\dot{\omega}}_b^d$) level (see Fig.\ref{fig:controller}). 
% %%
% %The desired (feed-forward) accelerations $\vc{\ddot{x}}^d$
% %are combined with feed-back accelerations produced by a virtual model and sent $\vc{\vc{\ddot{x}}^{ref}} =(\vc{\ddot{x}}_{cog}^{ref}$, $\vc{\dot{\omega}}_b^{ref})$ to the Inverse Dynamics algorithm.  
% %On the other hand, the swing leg joint torques are computed only by the PD controller.
% 
% %\sout{During execution the footsteps are
% %continuously re-planned and updated to account for inaccuracies in execution and
% %perception.} The following describes the modules of the controller in detail.
% 
% \subsection{Virtual Model}
% The feedback action which compensates for possible inaccurate execution and
% drift is created by a virtual spring and damper system as in
% \cite{Havoutis2014}. The linear/rotational springs map an error in
% position/orientation into a force $\vc{F}_{vm}$ and torque $\vc{T}_{vm}$ acting
% on the robot body (\fref{fig:virtual_model}) as:
% \begin{equation}
% \begin{aligned}
% 	& \vc{F}_{vm} = \mx{P}_x (\vc{x}_{com}^d - \vc{x}_{com}) + \mx{D}_x
% 	(\vc{\dot{x}}_{com}^d - \vc{\dot{x}}_{com})\\
% 	& \vc{T}_{vm} =  \mx{P}_{\theta} e(\mx{R}_b^d \mx{R}_b^\T) + \mx{D}_{\theta}
% 	(\boldsymbol{\omega}_b^d - \boldsymbol{\omega}_b),
% \end{aligned}
% \label{eq:virtual_model}
% \end{equation}
% where the superscript $d$ refers to the desired values dictated by the
% whole-body motion generator and non-superscript values describe the state of the
% robot as estimated by the on-board state estimator \cite{Bloesch12state}.
% We define $e(.): \Rnum^{3\times 3} \rightarrow \Rnum^3$ as a mapping from a
% rotation matrix to the associated rotation vector \cite{Caccavale1999}, and
% $\mx{P}_x, \mx{D}_x,\mx{P}_{\theta}, \mx{D}_{\theta}\in \Rnum^{3\times 3}$ as
% the positive-definite diagonal matrices of proportional and derivative gains,
% respectively. Expressing the body feedback action in terms of forces and moments
% allows us to give the virtual model gains a physical meaning of stiffness and
% damping and thus can be intuitively set and used.
% 
% Since the inverse dynamics computation requires reference
% \textit{accelerations}, we multiply the forces/moments (\textit{wrench})
% $\vc{\mathcal{W}}_{vm} = ( \vc{F}_ {vm}, \vc{T}_{vm})$ with the inverse of the
% composite rigid body inertia, $\mx{I}_c$, of the robot at its current
% configuration. Adding this body feedback acceleration to the desired body
% acceleration produced by the whole-body motion generator creates the 6D
% reference acceleration (linear/rotational) for the inverse dynamics computation
% as:
% \begin{equation}
% 	 \vc{\ddot{x}}^{ref}= \vc{\ddot{x}}^d  + I_c^{-1}\vc{\mathcal{W}}_{vm}.
% \label{eq:desired_acc}
% \end{equation}
% 
% By combining a feed-forward acceleration $\vc{\ddot{x}}^d$ with a body-feedback
% acceleration, we achieve accurate tracking while maintaining a compliant
% behavior. This is crucial for robots that physically interact with their
% environment, in real-world scenarios.
% 
% \begin{figure}[tb]
%   \centering
%   \includegraphics[width=0.6\textwidth]{figs/decoupled_planning/virtual_model.pdf}
%   \caption[A virtual model control scheme is used to close a feedback loop at
%   the robot-body level]{
%   A virtual model control scheme is used to close a feedback loop at
%   the robot-body level \citep{Havoutis2014}. Effectively, this is a PD tracking
%   controller that tries to minimize the error between the desired and current
%   body state (position and orientation). This produces the feedback wrench
%   ($\vc{\mathcal{W}}_{vm}$) that is then transformed to the feedback body
%   acceleration, $\vc{\ddot{x}}^{fb}$.}
%   \label{fig:virtual_model}
% \end{figure}
% 
% 
% \subsection{Floating- Base Inverse Dynamics}
% The floating-base inverse dynamics algorithm calculates the joint torques 
% required to execute the reference body accelerations. We can partition the 
% dynamics equation of the robot into the unactuated base coordinates $\vc{q}_b$
% ($n_b$ = 6 equations for our case) and the active joints' coordinates $\vc{q}_q$
% ($n_q$ = 12 equations),  e.g. \cite{Fujimoto1998}, as:
% %
% \begin{equation}
% 	\underbrace{\mx{H}(\vc{R}, \vc{q})  \mat{\vc{\ddot{q}}_b \\ \vc{\ddot{q}}_q} + 
% 	\mat{\vc{h}_b \\ \vc{h}_q }(\vc{R}, \vc{q}, \boldsymbol{\omega},
% 	\vc{\dot{q}})}_\vc{b} = \mat{\vc{0}\\ \boldsymbol{\tau}} + \mat{\mx{J}_{cb}^T\\
% 	\mx{J}_{cq}^T } \boldsymbol{\lambda},
% \label{eq:inverse_dynamics}
% \end{equation}
% where $\mx{H}$ is the floating-base mass matrix, $\vc{h} = (\vc{h}_{b},
% \vc{h}_{q})$ is the force vector that accounts for Coriolis, centrifugal, and
% gravitational forces, $\boldsymbol{\lambda}$ are the ground contact forces, and
% their corresponding Jacobian $\mx{J}_c = \mat{ \mx{J}_{cb} & \mx{J}_{cq}}$.
% $\boldsymbol{\tau}$ is the vector that holds the inverse-dynamics torques that
% are calculated.
% 
% The left hand term, $\vc{b} = (\vc{b}_{b}, \vc{b}_{q})$, can be computed
% efficiently using the Featherstone implementation of the \ac{RNEA}
% \cite{Featherstone2008}. Since the \gls{com} acceleration
% $\vc{\ddot{x}}_{com}^{ref}$ is defined in a frame aligned with the base frame
% but with the origin in the \gls{com}, a translational coordinate transform
% $_b\mx{X}_{com}$ is performed to get the 6D base spatial acceleration:
% $\vc{\ddot{q}}_b  =\,  _b\mx{X}_{com} \vc{\ddot{x}}^{ref}$, as in
% \cite{Featherstone2008}.
% 
% By partitioning the dynamics equation, as in \eqref{eq:inverse_dynamics}, and
% given that the base is not actuated, we can directly compute, in a least-squares
% way, the vector of ground reaction forces $\boldsymbol{\lambda}$ from the first
% $n_b$ equations, $\boldsymbol{\lambda} = \vc{J}_{cb}^+ \vc{b}_b$, where $()^+$
% denotes the Moore-Penrose generalized inverse. The last $n$ equations are used
% to produce the reference joint torques, $\boldsymbol{\tau}^{id} = \vc{b}_q-
% \mx{J}_{cq}^T\boldsymbol{\lambda}$.
% 
% 
% 
% \section{Results}\label{sec:decoupled_results}
% The following section describes the experiments conducted to validate the
% effectiveness and quantify the performance of our framework. The first set of
% experiments is designed to evaluate the capabilities of our motion planner. We
% use a set of benchmarks of realistic locomotion scenarios (see
% \cref{fig:planning_benchmarks}): stepping stones (top right), pallet (top left),
% stair (bottom right) and gap (bottom left). In these experiments, we compared
% the cost, number of expansions and computation time of \gls{aras} against
% \ac{A$^*$} using our lattice representation. The results are based on 9
% predefined goal locations. In the next experiment the robot must plan online
% with dynamic changes in the terrain. In the experiment that follows after, we
% show the online planning and perception results. Finally, we validate the
% performance of our locomotion framework with the \gls{hyq} robot.
% 
% \begin{figure}%[b]
% 	\centering
%  	\includegraphics[width=0.98\columnwidth]{figs/decoupled_planning/planning_benchmarks.pdf}
%  	\caption[The planning benchmarks used to analyze the quality of the produced
%  	plans]{
%  	The planning benchmarks used to analyze the quality of the produced
%  	plans. \textit{Top left}: stepping stones; \textit{Top right}: pallet;
%  	\textit{Bottom left}: stair; \textit{Bottom right}: gap.}
% 	\label{fig:planning_benchmarks}
% \end{figure}
% 
% 
% \subsection{Evaluation of path and foothold planning}
% \subsubsection{Initial plan results}
% The stepping stones, pallet, stair and gap experiments evaluate the initial plan
% quality (see \Cref{tab:results_plan}) of our approach using \ac{A$^*$} and
% \gls{aras}. To this end, we plan a set of body actions and foothold sequences
% between 9 predefined goal locations, approximately \unit[2]{m} away from the
% starting position, and compare the cost and number of expansions of the body
% action path, and the planning time of \gls{aras} against \ac{A$^*$}. Three
% main factors contribute to the decreased planning time while maintaining the
% quality of the plan:
% 
% First, the lattice-based representation (using body movement primitives)
% considers versatile movements in the sense that it allows us to reduce the
% search space around feasible regions (feasible motions) according to a certain
% body action, in contrast to grid-based approaches that ensure the feasibility by
% applying rules that are unaware to body actions. Second, our terrain-aware
% heuristic function guides the tree expansion according to terrain conditions in
% contrast to a simple Euclidean heuristic. Finally, the \gls{aras} algorithm 
% implements a search procedure that guarantees bounded sub-optimality in the
% solution given a proper heuristic function \cite{Likhachev2004}. 
% \cref{fig:compared_planning} shows the initial plan of \ac{A$^*$} and \gls{aras}.
% 
% The plans that \gls{aras} produces within the given time budget are on average
% twice as costly as the plans of \ac{A$^*$}. Nevertheless, this allows for a dramatic
% decrease of the time it takes to compute a path, \unit[333.9]{sec} for \ac{A$^*$}
% versus \unit[1.7225]{sec} for \gls{aras}, while any extra time budget can be used to
% optimize (\textit{repair}) the computed path. These results were obtained in
% the onboard PC on \gls{hyq}, i.e a Pentium i5 with Linux kernel. Note that
% \gls{aras} can be let to run until exhaustion, inc which it would match the
% characteristics in final path cost and computational time of \ac{A$^*$}.
% 
% \begin{figure}[!tb]
% 	\centering
%  	\includegraphics[width=0.75\columnwidth]%{figs/compared_planning_v.pdf}
%  	{figs/decoupled_planning/compared_planning_v.pdf}
% 	\caption[The body action (green line) and foothold sequence plan of
% 	\acs{A$^*$} (left) and \acs{ARA$^*$} (right) given the costmap (grey scale)]{
% 	The body action (green line) and foothold sequence plan of
% 	\acs{A$^*$} (top) and \acs{ARA$^*$} (bottom) given the costmap (grey scale).
% 	The brown, yellow, green and blue points represent the planned footholds of the
% 	\acs{LF}, \acs{RF}, \acs{LH} and \acs{RH} feet, respectively.}
% 	\label{fig:compared_planning}
% \end{figure}
% 
% \begin{table}[!b]
% 	\centering
% 	\caption{Cost of the plan (Cost), number of expansions (Exp.) and
% 	computation time (Time, in seconds) averaged over 9 trials of \acs{A$^*$} and
% 	\acs{ARA$^*$}.}
% 	\begin{tabular}{@{} lrrrrrr @{}}    
% 	\toprule 
% 	&\multicolumn{3}{c}{\acs{A$^*$}} & \multicolumn{3}{c}{\acs{ARA$^*$}} \\
% 	\cmidrule{2-4}\cmidrule{5-7}
% 	\emph{Terrain}	& Cost  & Exp. & Time  & Cost  & Exp. & Time \\
% 	\midrule
%  	S. Stones	  	& 364.7 & 3191 & 428.7 & 597.4 & 12.1 & 1.59 \\ 
%  	Pallet 			& 269.2 &  270 & 271.2 & 587.7 & 12.7 & 1.74 \\ 
%  	Stair  			& 306.1 &  306 & 308.1 & 646.4 & 12.7 & 1.55 \\
%  	Gap				& 325.6 &  326 & 327.6 & 647.0 & 13.0 & 2.01 \\
% 	\bottomrule
% 	\end{tabular}
% 	\label{tab:results_plan}
% \end {table}
% 
% \subsubsection{Online planning and perception}
% Using a movement primitive-based lattice search reduces the size of the search
% space significantly, leading to responsive planning and replanning the next set
% of steps. In our experimental trials, we chose a lattice graph resolution
% (discretization) of \unit[4]{cm} for $x/y$ and 1.8$^\circ$ for $\theta$ and goal
% state is never more that \unit[5]{m} away from the robot. In these trials, the
% plan/replan frequency is approximately \unit[0.5]{Hz}.
% 
% On the other hand, the efficient occupancy grid-based mapping allows us to
% incrementally build up the model of the environment and focus our computations
% to the area of interest around the robot body, generating plans quickly. This
% allows us to locally update the computed costmap and incrementally build the
% costmap as the robot moves with an average response frequency of \unit[2]{Hz}.
% 
% \begin{figure}%[!b]
% 	\centering
%  	\includegraphics[width=0.98\columnwidth]{figs/decoupled_planning/replanning}
% 	\caption[(Re-)planning and perception on-board]{
% 	(Re-)planning and perception on-board. The left image presents the
% 	plan for a flat terrain, then, the right image reflects the re-planning and
% 	updating of the costmap (grey scale map). The green, brown, blue and yellow
% 	points represent the planned footholds of the \acs{LH}, \acs{LF}, \acs{RH},
% 	\acs{RF} legs, respectively. The green line represents the body path according
% 	to action plan.}
% 	\label{fig:replanning}
% \end{figure}
% 
% We generate swift and natural dynamic whole-body motions from an n-step
% lookahead optimization of the body trajectory that uses a dynamic stability
% metric, the \gls{cop}. A combination of floating-base inverse dynamics and
% virtual model control accurately executes such dynamic whole-body motions with
% an actively compliant system \cite{Winkler2015}. Our locomotion system is robust
% due to a combination of online planning and compliance control, as presented in
% \Cref{sec:decoupled_execution}.
% 
% \begin{figure*}[htb]
% 	\centering
% 	\includegraphics[width=0.98\textwidth]{figs/decoupled_planning/planning_snapshots.png}
% 	\caption[Snapshots of pallet trial used to evaluate the performance of our
% 	planning approach]{
% 	Snapshots of pallet trial used to evaluate the performance of our
% 	planning approach. From top to bottom: planning and terrain costmap; execution
% 	of the plan in \acs{HyQ}.}
% 	\label{fig:planning_vidsnaps}
% \end{figure*}  
% 
% 
% \subsection{Trials}
% The first experiment starts with a flat, obstacle-free terrain. After the robot
% has planned initial footholds, a pallet is placed into the terrain
% (\cref{fig:replanning}). Later we show the terrain costmap, the planned
% footholds, and the execution of an initial plan in \cref{fig:planning_vidsnaps}.
% In the next experiments the robot must climb one and two pallets of dimensions
% \unit[1.2]{m}~$\times$~\unit[0.8]{m}~$\times$~\unit[0.15]{m}. The height of one
% pallet is equal to 20\% of the leg length. Furthermore we show that the robot
% traverses a gap of \unit[35]{cm}, which is approximately half the length between
% the front and hind hips. The final experiment consist of two pallets connected
% by a sparse path of stepping stones. The pallets are \unit[1.2]{m} apart and the
% stepping stones lie \unit[0.08]{m} lower than the pallets.
% 
% For each experiment, we specify the $\vc{s}=(x,y,\theta)$ goal state. The
% foothold planner finds a sequence of footsteps of an arbitrary order, which the
% controller then executes dynamically. We validate the performance of our
% framework in 4 scenarios as seen in \cref{fig:decoupled_vidsnaps} and compare it
% to our previously achieved results (\Cref{tab:decoupled_results}) on the same
% benchmark tasks. Additionally, \cref{fig:trial_over} shows an overview of the
% benchmark trials along with generated footholds and body motion plans.
% 
% \subsection{Evaluation of whole-body motion generation and
% execution}\label{sec:evaluation}
% We evaluate the performance of the our locomotion framework in few different
% point of view: perception and (re-)planning, speed while dynamically stable,
% model accuracy, avoiding kinematic limits and stability despite irregular
% swing-leg sequences. All these aspects evaluate individually the performance of
% the foothold and motion planner.
% 
% \begin{figure*}[tb]
%   \centering
%   \includegraphics[width=0.98\textwidth]{figs/decoupled_planning/vidsnaps/all_line_v.jpg}
%   \caption[Snapshots of 4 experimental trials used to evaluate the performance
%   of our framework]{
%   Snapshots of 4 experimental trials used to evaluate the performance
%   of our framework. From top to bottom row: crossing a \unit[15]{cm} hight
%   pallet; climbing a stair-like structure consisting of two stacked pallets;
%   traversing a \unit[35]{cm} gap and crossing a sparse set of stepping stones.
%   In addition, \fref{fig:trial_over} gives and overview of the chosen footholds,
%   planned body paths and executions on this set of benchmark trials.}
%   \label{fig:decoupled_vidsnaps}
% \end{figure*}  
% %
% \begin{table}[!t]
%   \caption{Forward speed and success rate of experiments averaged over 10 trials
%   and compared to previous results from \cite{Winkler2014}.}
%   \label{tab:decoupled_results} 
% \begin{center}
% \begin{tabular}{@{} lrrrrrrr @{}}
% \toprule
% &\multicolumn{3}{c}{Speed [cm/s] } && \multicolumn{3}{c}{Success Rate [\%]} \\
% \cmidrule{2-4}\cmidrule{6-8}
% \emph{Terrain} 	& Curr. &Prev. &Ratio &&   Curr. &Prev. &Ratio\\
% \midrule
%  Step. Stones  	&  7.3  &1.7   &4.2  &&   60    &70  &0.9      \\ 
%  Pallet 	    &  9.5  &2.1  &4.5   &&   100   &90  &1.1       \\ 
%  Two Pallets  	& 10.2  &1.8  &5.8   &&   90    &80  &1.1       \\
%  Gap			& 12.7  &\enspace- &\enspace- &&   90   &\,\,0   &\enspace-    \\
% \bottomrule
% \end{tabular}
% \end{center}
% \end{table}
% 
% \begin{figure}%[tb]
% \centering	
% \subfloat[Stepping over a pallet.]{\resizebox{0.85\columnwidth}{!}{
% \includegraphics{figs/decoupled_planning/trials/pallet_plot}}} \\
% \subfloat[Crossing a 35cm gap.]{\resizebox{0.85\columnwidth}{!}{
% \includegraphics{figs/decoupled_planning/trials/gap35_plot}}} \\
% \subfloat[Stair-climbing.]{\resizebox{0.85\columnwidth}{!}{
% \includegraphics{figs/decoupled_planning/trials/two_pallets_plot}}} \\
% \subfloat[Crossing a sparse set of
% stepping-stones.]{\resizebox{0.85\columnwidth}{!}{
% \includegraphics{figs/decoupled_planning/trials/stepping_stones_plot}}}
% 	\caption[Overview of experimental trials]{
% 	Overview of experimental trials. Filled circles represent 
% 	color-coded footholds, i.e. the brown, yellow, green and blue represent the
% 	\acs{LF}, \acs{RF}, \acs{LH} and \acs{RH} feet, respectively. The gray squares
% 	represent pallet and stepping-stone geometries. The solid blue line is the
% 	desired dynamically-stable body trajectory, while the red dashed line is the
% 	actual trajectory that the robot achieves. Possible reasons behind this
% 	difference are discussed in \Cref{sec:decoupled_discussion}.}
% 	\label{fig:trial_over}
% \end{figure}
% 
% \subsubsection{Perception and (re-)planning}
% Efficient occupancy grid-based mapping and focusing our computations to an area
% of interest around the robot body greatly increase computation speed. This allows
% us to incrementally build a model of the environment and update the terrain
% costmap at a frequency of \unit[2]{Hz}. Using the action-based search graph
% together with \gls{aras} allows us to replan footholds at a frequency of
% approximately \unit[0.5]{Hz} for goal states up to \unit[5]{m}.
% 
% \subsubsection{Speed while dynamically stable} 
% The pallet climbing and gap experiments show the \emph{speed}
% (\tref{tab:decoupled_results}) that our framework can achieve: This is due to
% the fact, that the body can move faster while still being stable, since we are
% using a \emph{dynamic} stability criterion. All accelerations and decelerations
% are optimized, so that the \gls{com} never leaves the support polygon. In
% addition, since we are not directly producing torques with the virtual model
% feedback controller, but only accelerations for the inverse dynamics controller
% our feedback actions also respect the dynamics of the system. Furthermore, the
% duration of the four-leg-support phase is significantly reduced: It is much
% faster to move the \gls{com} from one support triangle to another one.
% 
% \subsubsection{Model accuracy} 
% Walking over a \unit[35]{cm} gap (approximately half the length between front
% and hind hips) shows the stability of the robot despite of dynamic motions. When
% crossing the gap the robot accelerates up to a body velocity of \unit[0.5]{m/s} 
% and is able to decelerate again without losing balance. This shows, that the
% simple cart-table model is a sufficient approximation for large quadrupeds 
% performing locomotion tasks.
% 
% \subsubsection{Avoiding kinematic limits} 
% Attempting to cross the gap with a statically stable gait would overextend 
% the legs, since large body motions are required to move the robot into statically
% stable positions. Dynamic motions allow us to keep the \gls{com} closer to the 
% center of all four feet, since stability can be achieved by appropriate
% accelerations, avoiding kinematic limits.
% 
% \begin{figure}[!h]%[tb]
% 	\centering
% 	\subfloat[Stepping stones execution]{\resizebox{0.95\columnwidth}{!}{
% 	\includegraphics{figs/decoupled_planning/trials/cog_trajectory_real.pdf}
% 	\label{fig:cog_trajectory_real}}} \\
% 	\subfloat[Stepping stones plan]{\resizebox{0.95\columnwidth}{!}{						
% 	\includegraphics{figs/decoupled_planning/trials/cog_trajectory.pdf}
% 	\label{fig:cog_trajectory_des}}}
% 	\caption[The \acs{HyQ} robot when walking over the stepping stones]{
% 	(a) The body motion when walking over the stepping stones is 
% 	shown in black. The planned footholds are shown and the irregular step 
% 	sequence \acs{LF}(1)~$\rightarrow$~\acs{LH}(2)~$\rightarrow$~\acs{RF}(3) is
% 	highlighted (red circles). (b) The 3 shrunk support triangles corresponding to
% 	the highlighted step sequence brown~$\rightarrow$~green~$\rightarrow$~yellow are
% 	shown. Additionally the planned \acs{CoM} (solid line) and \acs{CoP} trajectory
% 	for the duration of these 3 steps is illustrated (asterisk). While the
% 	\acs{CoM} (solid line) does not reach the support triangles, the \acs{CoP}
% 	does, causing dynamic stability. When switching between disjoint support
% 	triangles (green~$\rightarrow$~yellow) four-leg support phases are inserted
% 	(red) to allow a smooth transition.}
% 	\label{fig:cog_trajectory}
% \end{figure} 
% 
% \subsubsection{Stability despite irregular swing-leg sequences} 
% Walking over the stepping stones demonstrates the ability of the controller to 
% execute irregular swing-leg sequences in a dynamically stable manner.
% \cref{fig:cog_trajectory} shows how starting from a lateral sequence gait
% (\ac{LH}-\ac{LF}-\ac{RH}-\ac{RF}) the foothold sequence changes to traverse
% these irregularly placed stepping stones. Despite this, the generated \gls{com}
% trajectory (colored solid line, bottom) is dynamically stable, since the
% \gls{cop} (asterisk) is always kept inside the current support triangle. When
% comparing the actual (top) and desired (bottom) \gls{com} trajectories, a
% tracking error is evident. By keeping the \gls{cop} e.g. $r =$ \unit[6]{cm} away
% from the stability borders, we are robust even against these inaccuracies.
% 
% The whole body motion generator inserts four-leg-support phases (red section)
% only whenever it detects disjoint support triangles in the swing-leg sequence.
% While executing steps 1 and 2 (\cref{fig:cog_trajectory}) no four-leg-support
% phase is necessary, because the triangles are not disjoint. Only after returning
% to swing the right-front leg, the robot requires a four-leg support phase for
% the \gls{cop} to transition from the green (\ac{LH}) to the yellow (\ac{RF})
% support triangle at $(x,y)=(1.1, 0)$.
% 
% 
% 
% \section{Discussion}\label{sec:decoupled_discussion}
% In this section we will identify possible factors that can limit the success of
% our framework (failures). This is according to the trials that we have performed
% over a substantial period of working with the \gls{hyq}.
% 
% (\textit{1}) The \textit{cart-table model} estimates the \gls{cop} position but
% neglects the angular components of the motion of the body which can lead to
% inaccurate evaluation of the \gls{cop} within the support polygon. This does not
% affect the behavior when the attitude of the robot does not change but can
% affect stability going up or down stairs, crossing uneven stepping stones, etc.,
% and the body trajectory changes along roll, pitch and yaw. In practice \gls{hyq}
% never generates angular body accelerations that can move the \gls{cop} that far
% away from the simplified estimate point. In addition the stability margin, $r$,
% that is defined inside the support polygon, ensures that error in estimation,
% model inaccuracies or the use of the simplified \gls{cop} measure, do not impact
% the robot's stability. \Cref{sec:preview_generation} will present a methodology
% to guarantee dynamic walking with trunk attitude modulation.
% 
% (\textit{2}) Unwanted \textit{foot-slippage} can impact the performance of our
% framework. This can happen when the acceleration of the body is significant and
% one or some of the feet slip backwards, or when a foot is only slightly loaded
% so subsequent ``pushing" backwards results in the foot sliding. The former
% occurs due to non-explicitly-bounded body acceleration at the body trajectory
% optimization phase and due to no friction-cone constraints in the inverse
% dynamics torque calculation step. The latter is also attributed to the lack of
% friction-cone constraints at the inverse dynamics torque calculation, while
% setting a minimum loading threshold, i.e. a minimum loading value beyond which
% to consider a leg as in stance, can solve this problem. In practice this limits
% the forward velocity that can be achieved by the framework, as large
% accelerations can result in slippage, and limit behaviors within conservative
% bounds. Approaches that include friction-cone constraints can be applied. In the
% next chapter we show a \ac{QP}-based optimization of inverse dynamics, that
% limits the \ac{GRFs} within the estimated friction-cone approximations and
% ensures adequate loading for all stance legs as presented in \cite{Focchi2016}.
% 
% (\textit{3}) Last, accurately estimating the state of the robot has also proven 
% a challenging task. An adequately reliable state-estimate is important for 
% executing planned walks, as foot placement directly depends on the estimate of
% the body position. In addition, the body-level feedback loop that the \ac{VM} 
% implements also depends on the body state estimate. This estimate generally
% slowly drifts in yaw, something that affects the position estimate and 
% subsequently distorts the maps created over a longer time period. Using vision
% approaches can eliminate drift and improve the state estimate but up to now this
% has been beyond the scope of our research. Currently we have been working in the
% developing of state estimation algorithms for quadrupedal locomotion over rough
% terrain \citep{Camurri2016}. Another source of state estimate error is
% foot-slippage, as the algorithm used assumes that stance feet do not move with
% respect to the world frame. This can produce sudden jerks that can affect the
% inverse dynamics loop and also cause the position estimate to drift. We believe
% that by alleviating the foot-slippage problem we would also considerably
% increase state estimation accuracy.
% 
% 
% 
% \section{Conclusion}\label{sec:decoupled_conclusion}
% In this chapter, we presented a dynamic whole-body locomotion framework that
% executes versatile movements that are planned on-board. We showed, how sequences
% of footsteps are planned given a body action plan, and how a change in the
% environment causes the foothold generator to replan footholds online. We used
% a set of predefined body movement primitives to reduce the computational demand
% of planning, and compute plans online using incoming terrain information.
% We presented a whole body motion planner, which is able to generate a
% \gls{cop}-stable body trajectory despite irregular swing-leg sequences to
% execute footholds dynamically.
% 
% Decoupling motion and foothold planning increase the computation time by
% reducing the search space. In these approaches, the foothold selection can just
% consider the robot's kinematic model, which limits the locomotion capabilities
% of our system (e.g. step time modulation). As a consequence the dynamic
% trajectory generator requires to tune an appropriate step time given a foothold
% sequence. Furthermore, the foothold planning may not be able to plan for more
% complex terrain conditions such as stepping stones with fewer stones. In
% \Cref{sec:coupled_planning}, we show how a coupled motion and foothold planning
% approach increases the capabilities of the locomotion system. This planning
% approach adapts the step duration and can tackle more complex stepping stones
% terrains.
% 
% The cart-table model reduces the dimensionality of the problem but neglects the
% angular momentum of the motion, which is required for climbing up and down
% tasks. However, our experiments show that we can tackle terrain with small
% elevation with the cart-table model. In \Cref{sec:preview_generation} we develop
% a novel method that ensures dynamic stability (i.e. the \gls{cop} condition)
% while the trunk attitude is adapted. For that, the stability margin is used to
% allow the robot to limit the trunk attitude adjustment. We limit the trunk
% attitude accelerations because it allows us to bound the maximum applied
% \gls{com} torque. In fact, this will limit the difference between the \gls{cop}
% and \ac{CMP} points. And as result the \gls{cop} condition cannot guarantee
% dynamic stability if the \ac{CMP} does not stay inside the support polygon.
% 
% The discretization of the terrain model shows good performance in terms of
% foothold selection and computation time. We could represent the different
% terrain benchmark with the aforementioned geometric features: standard deviation
% of height values, the slope and the curvature. Furthermore, a terrain model as
% costmap is a suitable description for motion planning in rough terrain as shown
% in other works \citep{Kolter2008b}\citep{Kalakrishnan2010b}\citep{Winkler2014}.
% Other ways of modeling the terrain can be implemented with constraint but they
% might increase the complexity of problem. Furthermore, the terrain costmap might
% not be a convex function, which increases the problem complexity.
% \Cref{sec:preview_optimization} presents a method that addresses these issues.
% 
% In the next chapter, we bring the kinematic planning (i.e. foothold planner) and
% the dynamic execution closer. The idea is to produce desired state trajectories
% and footholds through a \emph{single} trajectory optimization problem (i.e. coupled
% planning). Additionally, we develop a \ac{QP}-based controller where it ensures
% that the \ac{GRFs} respect the friction-cone constraints.


==> src/terrain_server.tex <==
\section{Terrain mapping}\label{sec:terrain_mapping}
This section describes the pipeline of acquisition and evaluation of terrain
information. We implemented an onboard terrain information server that holds and
continuously updates the state of the environment. We show how this information
is processed and transformed to a qualitative metric of the terrain topology.

\begin{figure}[b]%[!tb]
	\centering
	\href{http://youtu.be/yrEOE0pZMlc}{\includegraphics[width=0.95\columnwidth]{figs/terrain_server/terrain_voxelmap-compressed}}
	\caption[The \gls{hyq} robot mapping the terrain using Octomap
	\citep{Hornung2013}]{
	The \gls{hyq} robot mapping the terrain using Octomap \citep{Hornung2013}.
	The	voxel map is generated from RGBD camera data (Asus Xtion), using the
	estimated
	body position. The RGBD sensor is mounted on a \gls{ptu} that scans the
	terrain, with a left/right sweep and up/down frequency of \unit[1]{Hz}. The
	occupancy map is built with a \unit[2]{cm} resolution. To watch the video,
	click the figure.}
	\label{fig:terrain_voxelmap}
\end{figure}

An occupancy map holds the 3D geometric perception data scanned from vision
sensors mounted at the front of the robot (see \Cref{fig:terrain_voxelmap}).
For that, we use Octomap\footnote{The source code is available on
\href{https://github.com/OctoMap/octomap}{https://github.com/OctoMap/octomap}.}
as this provides a probabilistic representation that handles sensor noise.
Octomap represents both free and occupied spaces and satisfies the required
computation time for our application, which is at least \unit[2]{Hz} with
onboard
processing (see \sref{sec:results} for details about the onboard PCs). Octomap
uses a hierarchical data structure, for spatial subdivision in 3D, called
\textit{octrees}. This octree-based representation is designed to efficiently
update and copy the map \citep[for more details see][]{Hornung2013}. Moreover,
it has a multi-resolution volumetric representation that we use to speed up the
computation time of the geometric features such as \textit{slope} and
\textit{curvature}.

% We use a \unit[2]{cm} resolution occupancy map because we found out
% that it is sufficient for the estimation of the features values, and it allows
% us to build online terrain costmaps (\Cref{sec:terrain_costmap}).

% We use a terrain information server to hold the geometric perception data and
% simplify the access to terrain information queries. The required information for
% the motion planning, e.g. the \textit{terrain costmap} and the \textit{terrain
% heightmap} of the environment around the robot, is computed based on the
% information that this server holds. We


\subsection{Terrain costmap}\label{sec:terrain_costmap}
The \textit{terrain costmap} quantifies how desirable it is to place a foot at a
specific location. The cost value for each voxel in the map is computed using
geometric terrain features such as \textit{height deviation}, \textit{slope}
and \textit{curvature} \citep[similar to][]{Kolter2009}. We compute the
slope and curvature through regression in a \unit[6]{cm}$\times$\unit[6]{cm}
window around the cell in question; the features are computed from a voxel model
(\unit[2]{cm} voxel-size resolution) of the terrain. For instance, the estimated
surface normals and curvatures are computed from a set of neighboring occupied voxels.
We estimate the surface normals through an analysis of the eigenvectors and
eigenvalues, a procedure using \gls{pca}, of the set of nearest neighbors (for more
information, including the mathematical equations of the least-squares problem,
see \citep{RusuThesis}). Each surface normal is computed from the
eigenvector that has the smallest eigenvalue, $\lambda_0$ and the surface
curvature $\sigma$ as follows:
\begin{equation}\label{eq:curvature}
	\sigma = \frac{\lambda_0}{\lambda_0 + \lambda_1 + \lambda_2}
\end{equation}

\begin{figure}[b]%[!tb]
	\centering
	\href{http://youtu.be/a_H7pwCpi0g}{\includegraphics[width=0.95\columnwidth]{figs/terrain_server/normal_vector_field_v2-compressed}}
	\caption[A set of surface normals are extracted from the RBGD sensor]{
	A set of surface normals are extracted from the RGBD sensor. The surface
	normals are estimated from the eigenvalues and eigenvectors computed from the
	nearest neighbors of a query point. To watch the video, click the figure.}
	\label{fig:normal_vector}
\end{figure}

\cref{fig:normal_vector} shows a set of estimated surface normals from
the occupancy map of a cobblestone terrain. We compute the normals, and other
geometric features, with \unit[2]{cm} of resolution (i.e. costmap resolution).
We build the terrain costmap on top of the occupancy map; therefore, the terrain
map has its own voxel-size resolution. For all terrain costmaps in this article
we use a resolution of \unit[2]{cm}.

The terrain costmap is incrementally built based on the aforementioned features
and updated locally whenever a change in the map is detected. For computing the
terrain costmap, we define an area of interest around the robot of
\unit[2.5]{m}$\times$\unit[5.5]{m}. For each pixel of the terrain map, the cost
value is computed as a weighted linear combination of the individual features
$T(x,y) = \vc{w}^T \vc{T}(x,y)$, where $\vc{w}$ and $\vc{T}(x,y)$ are the
weights and feature cost values, respectively. The total cost value is
normalized, where 0 and 1 are the minimum and maximum cost values, respectively.
The weight vector describes the importance of the different features. We will
now give a brief overview of the different geometry features used for computing
the terrain cost values.

\subsubsection{Height deviation}
%$\\ $ %I need to do this to create a new line 
The height deviation cost penalizes footholds close to large drop-offs; for
instance, this cost is needed for crossing gaps or stepping stones. In fact,
staying far away from large drop-offs is beneficial because inaccuracies in the
execution of footsteps can cause the robot to step into gaps or banned
areas. For example, the \gls{hyq} robot foothold inaccuracies are around
\unit[4]{cm} (or 2 voxels) when slippage does not occur; note that
slippage events can increase the execution inaccuracies\footnote{Slippages
produce a drift in the estimated body position, for more details see
\cite{Camurri2017}.}. In addition, the height deviation cost also keeps the feet
away from areas in which the shin can collide with the environment, similar as
in \cite{Mastalli2015}. This is useful in climbing up/down stairs. The height
deviation feature $f_h$ is computed using the standard deviation around a
defined neighborhood.

\subsubsection{Slope}
%$\\ $ %I need to do this to create a new line 
The slope reflects the local surface normal in a neighborhood around the cell,
the normals are computed using \gls{pca} on the set of nearest neighbors. A high
slope value will increase the chance of slipping even in cases where the
friction cone is considered, e.g. due to inaccuracies in the friction
coefficient or estimated surface normal. Slope cost increases for larger slope
values, while small slopes have zero cost as they are approximately flat.
We consider the worst possible slope $s_{max}$ occurs when the terrain is very
steep (approximately 70$^{\circ}$)\footnote{We heuristically defined this value
based on our experience with the \gls{hyq} robot.}.

We map the height deviation and slope features into cost values through the
following piecewise function:
\[
T_f(x,y) =
\begin{cases}
  0  											   &	f\leq f_{flat} \\
 -\ln\Big(1-\frac{f(x,y)}{f_{max}-f_{flat}}\Big) &	f_{flat} < f < f_{max} \\
 T_{max}										   &	f\geq f_{max}
\end{cases}
\]
where $f_{flat}$ is a threshold that defines the flat conditions, $f_{max}$ the
maximum allowed feature value, and $T_{max}$ is the maximum cost value. In
\tref{tab:terrain_values} we report the used values for all the experiments.

\begin{table}[t]
  \centering
  \caption{Parameter values of the height deviation and slope cost functions.
  We use the same values for all the experiments presented in this work.}
  \begin{tabular}{rccc}
  \toprule
                              & $f_{flat}$      & $f_{\max}$            & $T_{\max}$\\\cmidrule{2-4}
    \textbf{height deviation} & 0.01            & 0.06                  & 1\\
    \textbf{slope}            & $\frac{\pi}{180}$ & $\frac{70\pi}{180}$ & 1\\
    \bottomrule
  \end{tabular}
  \label{tab:terrain_values}
\end{table}

\subsubsection{Curvature}
%$\\ $ %I need to do this to create a new line 
The curvature describes the stability of a given
foothold location. For instance, terrain with mild curvature (curvature between
$c = 6$ to $c = 9$) is preferable to flat terrain since it reduces the
possibility of slipping, as it has a bowl-like structure. Thus,
the cost is equal to zero in those conditions. On the other hand, high and low
curvature values represent a narrow crack structure in which the foot can get
stuck in ($c > 9$) or edge structure in which the foot can slip ($c < -6$),
respectively; in those conditions, we have a higher cost value.
We use the following piecewise function to compute the cost value from a
curvature value $c$:
\[
T_c(x,y) =
\begin{cases}
  0 															   &    c_{mild}^+ > c > c_{mild}^- \\
  T_{max}  										   			 	   &	c\leq c_{crack} \\
  																   &    c\geq c_{mild}^+ \\
  T_{max} - \ln\Big(\frac{c(x,y)-c_{low}}{c_{high}-c_{low}}\Big)   &	c_{crak} < c < c_{mild}^-
\end{cases}
\]
where $c_{crack} = -6$, $c_{mild}^- = 6$, $c_{mild}^+ = 9$ and $c_{\max} = 9$.

\cref{fig:terrain_costmap} shows the computation of the terrain costmap, using
the above-mentioned mapping between geometry features to cost values, from the
onboard RGBD sensor. The cost values are represented using a color scale, where
blue is the minimum cost and red is the maximum one.

\begin{figure}%[!tb]
	\centering
	\includegraphics[width=0.95\columnwidth]{figs/decoupled_planning/terrain_costmap-compressed}
	\caption[A costmap generatef from RGBD data]{
	A costmap generated from RGBD data. The occupancy map is
	built with a \unit[2]{cm} resolution. Then the set of features is computed
	and	the total cost value per voxel is calculated. 
	In addition, a heightmap is created with a resolution of \unit[2]{cm} in z.
	The cost values are represented	using a color scale, where blue is the
	minimum cost and red is the maximum.
	(Figure taken from \cite{Mastalli2015})}
	\label{fig:terrain_costmap}
\end{figure}


\subsection{Terrain heightmap}\label{sec:terrain_heightmap}
The terrain \textit{heightmap} allows the robot to define the vertical
component (i.e. z-direction) of the footstep. Indeed the trunk/swing trajectory
can be approximately planned to place the foot at the correct height. A higher
resolution of the heightmap helps the robot to accurately establish a footstep,
which improves the overall execution. The heightmap is computed using the same
resolution (\unit[2]{cm}) as the costmap in the $(x,y)$-plane. Along the
$z$-direction we desire higher accuracy to step safely onto obstacles, so we use
a resolution of \unit[1]{cm}. In essence, the heightmap is a
$2{}^{1}\!/_{2}$-dimensional \textit{projection} of the costmap that can be more
efficiently handled by the subsequent steps of the motion and foothold planning.
For instance, the terrain costmap associates the cost value to the highest
occupied voxel.

